Learning Data-Efficient Rigid-Body Contact Models: Case Study of Planar Impact

In this paper we demonstrate the limitations of common rigid-body contact models used in the robotics community by comparing them to a collection of data-driven and data-reinforced models that exploit underlying structure inspired by the rigid contact paradigm. We evaluate and compare the analytical and data-driven contact models on an empirical planar impact data-set, and show that the learned models are able to outperform their analytical counterparts with a small training set.

==> section_4_original/Data_driven.tex <==
\section{Data-Driven Contact Models} \label{sec:data-driven-models}
Sec.~\ref{sec:3.2} highlights the variability in optimal contact parameters across experiments, and indicates that a significant portion of the imparted impulses do not lie in the predictive range of the commonly used contact models. The analytical contact models rely on parametrization and introduction of additional constraints to generate subsets of the admissible imparted impulse to the object. As \citet{chatterjee1997rigid} discusses, the parameters used are only very coarse approximations to very complicated and difficult to model phenomena, and there is no reason to expect that these or the constraints imposed on the interactions are physically relevant.

In light of this, we propose three data-driven contact model formulations. The first class uses Gaussian Processes (GPs) to directly learn impulses in the Energy Ellipse (as opposed to analytical contact models which try to parameterize a subspace of Energy Ellipse). The second class uses GPs to select the best parameters for a contact model for each impact. The third class uses GPs to predict predict instantaneous wrench (linear force and torque), thereby relaxing the assumption that only a linear impulse is permitted.

\subsection{Data-driven Model Formulation - Class I} \label{sec:data-driven}
The contact model representation posed in Eq.~\ref{eq:2.1} can be learned directly from the data using the feature space:
\begin{align}
    \mathcal{X} = \{m,I,r_x,r_y,\vect{q},\vect{v}\}^i
\end{align}
and treating $\mathcal{Y} = \{\vect{q},\vect{v}\}^f$ as the output (dependant) space. Using this feature space gives the learned models a large amount of flexibility at the cost of dimensionality of the space (10-D). For impacts that are near rigid we can exploit the structure and assumptions of rigid body contact to reduce the dimension of the feature space. Consider Eq.~\ref{eq:2.5}, the Energy Ellipse demarcates the region in space for all feasible imparted impulses under the rigid-body assumption that satisfy the law of conservation of energy. This space is a function of the effective inertia at the contact point ($\mat{M}_c$) which encapsulates the position of the center of mass with respect to the contact point as well as the inertia of the object, and the velocity of the contact point $v_c$. As such we propose two feature spaces that exploit this structure:
\begin{align}
    \mathcal{X}_1 &= \{\mat{M}_{c,11},\mat{M}_{c,12},\mat{M}_{c,22},\vect{v}_{c,1},\vect{v}_{c,2}\} \\
    \mathcal{X}_2 &= \{(\mat{M}_c \vect{v}_c)_t,(\mat{M}_c \vect{v}_c)_n\} \\
    \mathcal{Y} &= \{P_t, P_n \}
\end{align}
Here $\mathcal{X}_1$ and $\mathcal{X}_2$ are respectively 5- and 2-D, a significant reduction from the 10-D space. $\mathcal{X}_5$ attempts to capture the key features required to reconstruct the space of admissible impulses, while $\mathcal{X}_2$ is a coarse approximation of this space, where only the tangential and normal momenta of the contact point are considered. To learn the contact models, we used Gaussian Processes (GPs) (\cite{rasmussen2006gaussian}) with an Automatic Relevance Determination (ARD) Square Exponential Kernel. We use this kernel to compensate for the relative differences in magnitudes of the features. 

\subsection{Data-driven Model Formulation - Class II} \label{sec:4.2}
The models presented in sec.~\ref{sec:data-driven} are able to make predictions that span a larger subspace of the Energy Ellipse than their analytical counterparts, but can conceivably produce infeasible predictions until trained on a sufficient number of data. This property may be undesirable in instances such as robotic locomotion, where a bad prediction may be catastrophic. In contrast, analytical models by construction produce feasible predictions for reasonable choices of parameters. To exploit the best of both worlds, we propose two formulations, i) Using an analytical model and learning the residual errors in prediction using a GP, and ii) Learning the correct choice of model parameters given pre-impact states, and using an analytical model to make the predictions. In both cases we use feature space $\mathcal{X}_2$ and the same kernels as sec.~\ref{sec:data-driven}.

\subsection{Data-driven Model Formulation - Class III}
The formulations proposed in sec.~\ref{sec:data-driven} and \ref{sec:4.2} both assume an instantaneous impact with no deformation, leading to a point contact and a linear impulse. Most practical systems exhibit some compliance and contact is usually over a patch with non-uniform pressure distribution. As a proxy to deformation and patch contact, we train a model on the same feature set as \ref{sec:data-driven} but on $\mathcal{Y}=\{P_t, P_n, \tau \}$, where $\tau$ denotes an impulsive torque. We add this extra degree of freedom to capture some of the detail missed by the previous classes and analytical models. 

\subsection{Data-driven Model Performance}

Fig.~\ref{fig:4.1} shows the performance of the data-driven models compared to the Best Post Hoc model (best performance of the analytical models) and the IRB Bound model (best performance of any rigid-body contact model). Both Class I and II are able to outperform the Best Post Hoc model, but only approach the IRB Bound model. These models are able to outperform their analytical counterparts, but because they are built using the same features and assumptions as the analytical models, they will not be able to exceed the IRB bound. In Class I, the $\mathcal{X}_5$ shows a marginally better performance over $\mathcal{X}_2$, as it has a richer description of the impact event. 

Fig.~\ref{fig:4.2} shows the expectation over the $\ell_2$-norm error in predicting the center of mass velocity as a function of the number of data used in the training. As expected, the Best Post Hoc (analytical models) is the worst performing, and the Class I and II lie between the Best Post Hoc and IRB Bound. Here we only show the best performing approach from each Class for brevity. Class III surpasses the performance of the IRB Bound significantly due to the added expressibility afforded by the wrench as opposed to the linear impulse. The number of data required to learn the models is fairly small, Class I and II converge within 100 trials, but Class III requires about 250 trials.

\begin{figure}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{section_4/model_gp_norm_1}
            \caption[]%
            {{\small Class I models.}}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{section_4/model_data_aug.pdf}
            \caption[]%
            {{\small Class II models.}}    
            \label{fig:mean and std of net44}
        \end{subfigure}
        \caption[ Data-driven contact models: the Gaussian Process regression results. ]
        {\small Data-augmented contact models: the AP Newton model is used as the analytical model and each data GP is trained with 450 examples.}
        \label{fig:4.1}
\end{figure}

\begin{figure}
        \centering
        \includegraphics[width=0.7\textwidth]{section_4/performance.pdf}
        \caption[]{Data-augmented contact models: the AP Newton model is used as the analytical model and each data GP is trained with 450 examples.}
        \label{fig:4.2}
\end{figure}


\section{Discussion \& Conclusion} \label{sec:conc}
Contact models fulfill an important role in robotics and are used extensively in locomotion \cite{kuindersma2016optimization} and manipulation \cite{ChavanDafle2015a}, yet the literature contains little work in empirical evaluation and comparison of the models prevalent in the field \cite{todorov2012mujoco}. In this paper we show that empirical data play an important role in highlighting the limitations of analytical models, and allowing construction of data-driven contact models that are able to outperform their analytical counter-parts. We also demonstrate that by exploiting known structure and assumptions about physical interactions, we can build models that are more data-efficient. In particular, here we were able to reduce a 10-D space to 5-D. We further show that significant improvements can be made to a models predictive ability by allowing a small amount of flexibility in its expressibility. 

The challenge with using a purely data-driven model is the potentially poor or infeasible predictions made by these models before being trained on enough data and without strong priors. In contrast, augmenting analytical contact models with data allows for feasible predictions with adjustments made as more data is collected, but the predictions rely on the prior generated by the these models, which may not be accurate. In applications such as locomotion where feasible priors are necessary, we could start with a model from Class II and as data is collected, switch to Class I or III. 

The present study focuses on the impact of a single object, and learns a contact model suitable for the predictions of outcomes. Two interesting questions to ask are: how well does the model learned for this object work in making predictions for other objects of different shapes and physical properties? Is it possible to use this model as a prior and learn a correcting model with far fewer samples? We can draw an analogy of this idea and that used in the computer vision community where pre-trained networks are often used as a starting point.
